Finding a Bounded-Degree Expander Inside a Dense One

It follows from the Marcus-Spielman-Srivastava proof of the Kadison-Singer conjecture that if $G=(V,E)$ is a $\Delta$-regular dense expander then there is an edge-induced subgraph $H=(V,E_H)$ of $G$ of constant maximum degree which is also an expander. As with other consequences of the MSS theorem, it is not clear how one would explicitly construct such a subgraph. We show that such a subgraph (although with quantitatively weaker expansion and near-regularity properties than those predicted by MSS) can be constructed with high probability in linear time, via a simple algorithm. Our algorithm allows a distributed implementation that runs in $\mathcal O(\log n)$ rounds and does $\mathcal O(n)$ total work with high probability. The analysis of the algorithm is complicated by the complex dependencies that arise between edges and between choices made in different rounds. We sidestep these difficulties by following the combinatorial approach of counting the number of possible random choices of the algorithm which lead to failure. We do so by a compression argument showing that such random choices can be encoded with a non-trivial compression. Our algorithm bears some similarity to the way agents construct a communication graph in a peer-to-peer network, and, in the bipartite case, to the way agents select servers in blockchain protocols.

==> trunk/expansion_proof.tex <==
\subsection{The compressed representation: Full description}
We next show that the probability that \ALG\ on the input graph $G$ completes
within $T$ rounds returning a graph $H$ which is not not an $\freq$-expander is
$\bigO(n^{-\beta})$ for a constant $\beta$.

To this purpose, we proceed as follows. Assume again that $R\in\{0,
1\}^{ndT\log\Delta}$ is an initial randomness configuration, corresponding to
an execution terminating within $T$ rounds with a non $\freq$-expanding graph
$H$. We prove that, if this is the case, we can produce a new lossless
configuration $R'$, such that $R'$ provides the same information as $R$, but
has length $ndT\log\Delta - \Omega(\log n)$ bits. This is enough to prove the
claim.\footnote{Note that the ``bad events" we are encoding are of the form
``\ALG\ stabilizes within $T$ rounds'' {\sc and} ``The resulting graph $H$ is
not an $\freq$-expander''.  If we consider $T = \bigO(\log n)$, together with
Lemma~\ref{lem:termination} this is enough to prove
Theorem~\ref{thm:main-expanders}.}

We use the following notation throughout the remainder of this proof.  For a
node $v\in S$, we denote by $\out_v$ the fraction of $v$'s edges in $E$ that
have an end-point in $V - S$, i.e., $|e(v, V - S)| = \out_v\Delta$. We denote
by $\freq_v$ the fraction of $v$'s accepted link requests (so edges of subgraph
$H$) with end-points in $V - S$. We further let $\out = \frac{1}{s}\sum_{v\in
S}\out_v$ and $\freq = \frac{1}{s}\sum_{v\in S}\freq_v$. 

To realize the compressed representation claimed above, we need the following
notions.
 
\begin{definition}\label{def:critical}
We say that a node $w$ is {\em semi-saturated at round $t$} if the number of
accepted incoming connection up to round $t-1$, plus the number of requested
connection at round $t$ from nodes in $V-S$ is at least $cd/2$. We say that a
node $w$ is {\em critical at round $t$} if it is not semi-saturated at round
$t$ but it has more than $cd$ connections (accepted or requested) at round
$t$.\footnote{Note that this implies that $w$ received more than $cd/2$
requests from $S$ at round $t$.}
\end{definition}

We make use of the following facts.

\begin{claim}\label{cl:saturated}
For every round $t$, the number of semi-saturated (resp. critical) 
nodes is at most $2n/c$ (resp. $n/c$).
\end{claim}
\begin{proof}
Consider a node that is semi-saturated at round $t$. This node was the
recipient of at least $cd/2$ link requests, that it either accepted {\em
before} round $t$, or it received in round $t$.  Since, from the definition of
\ALG, for every node, the overall number of its link requests that are accepted
within round $t-1$, plus the number of link requests it issues at round $t$
cannot exceed $d$, we have a total of at most $dn$ such requests over the
entire network. This immediately implies that the number of semi-saturated
nodes at round $t$ cannot exceed $2n/c$.  The argument for the number of
critical nodes at round $t$ proceeds along the same lines and is omitted for
the sake of brevity.
\end{proof}

\subsubsection{Compressed encoding and correctness}
In the paragraphs that follow, we describe how the evolution of the protocol is
encoded in the presence of a non-expanding subset $S$ (with $|S| = s\le n/2$
without loss of generality). We also show correctness of our encoding,
discussing how the original information can be recovered from the compressed
encoding, at least in those cases where this is not obvious.

\paragraph{Set $S$.} We represent $S$ by writing the number $s:= |S|$ in a
prefix-free way using $2\log s$ bits, and then writing the number $k$ such that
$S$ is the $k$-th set of size $s$ in lexicographic order, which takes $\log {n
\choose s}$ bits. In total, the cost to encode $S$ is
\begin{equation}
\label{reps}
2\log s + \log {n \choose s} \, .
\end{equation}


\paragraph{Requested connections originating from $S$ that are accepted.} For
each node $v\in S$, we write, in a prefix free way, the number $\ell_v$, using
$2\log \ell_v$ bits. Then we specify, within the first $\ell_v$ random choices,
the $d$ ones that correspond to accepted requests.\footnote{Again we encode the
integer $i$, such that the $d$ accepted requests correspond to the $i$-th
subset of requests of size $d$.} The overall cost incurred is 
\begin{equation}
\label{repaccs}
\sum_{v\in S} 2 \log\ell_v + \log {\ell_v \choose d} \, .
\end{equation}

\paragraph{Randomness of nodes in $V-S$.} We represent the randomness of nodes
in $V-S$ as it is, with no gain or loss.

\paragraph{Subset of accepted connections from $S$ to $V-S$.} For each node
$v\in S$, recall that $\epsilon_v d$ is the number of outgoing edges from $v$
into $V-S$. We represent the subset of accepted requested that do so, using the
same encoding used above. In total, our cost is
\begin{equation}
\label{repcut}
 \sum_{v \in S} 2 \log (\epsilon_v d) + \log {d \choose \epsilon_v d } \, .
\end{equation}

\paragraph{Destinations of accepted requests originating from $S$.} For each
node $v\in S$, we represent accepted connections to $V-S$ as they are (i.e.,
using $\log\Delta$ bits), with no gain or loss.  Connections with destination
in $S$ can be represented using $\log((1 - \out_v)\Delta)$ bits instead of
$\log\Delta$. Overall, the cost we incur is
\begin{equation}\label{reprandacc}
\sum_{v\in S}(1 - \freq_v)\nreq\log ((1 - \out_v)\Delta) 
+ \sum_{v\in S}\freq_v\nreq\log\Delta \, .
\end{equation}
Note that, to represent the destinations of a generic node $v$'s accepted
requests, we would use $\nreq\log\Delta$ bits without any compression. 

\paragraph{Subset of semi-saturated nodes at each step.} From its definition,
the set of semi-saturated nodes needs not be represented explicitely. In fact,
for every round $t$, this set is uniquely determined from the evolution of the
protocol up to round $t-1$ and the requests from nodes in $V - S$ at round $t$,
whose randomness is represented as it is.

\paragraph{Subset of critical nodes at each step.} Let $C_t$ be the set of
critical nodes at round $t$ and $c_t:= |C_t|$. We represent all such sets. This
costs us
\begin{equation}
 \label{repcrit}
 \sum_{t=1}^T 2\log c_t + \log { n \choose c_t }  \, .
\end{equation}

\paragraph{Destinations of rejected requests originating from $S$.} To
compress the representation of these choices, we leverage Claim
\ref{cl:saturated}. Specifically, for each node $v$, at each round $t$, we
represent each rejected connection going to a critical node using $\log c_t$
bits, and each other rejected connection, which necessarily goes to a
semi-saturated node, using $\log 2n/c$ bits. Let $\rc_t(v)$ be the number of
rejected connection requests from $v$ to critical nodes in round $t$, and
$\rss(v)$ be the number of rejected connection requests from $v$ to
semi-saturated nodes, over the whole process. Overall, this costs us
\begin{equation}
 \label{reprandrej} \sum_{v\in S} \left( \   (\ell_v - d ) + \left( 
 \rss(v) \cdot \log \frac{2n}{c}\right) + \left(  \sum_{t=1}^T \rc_t(v) \cdot  
 \log c_t \right) \ \right) \, .
\end{equation}

\paragraph{Unused randomness.} For every node $v$, we have enough randomness to
describe exactly $dT$ choices. If $v$ completes its execution of the protocol
after performing $\ell_v$ requests, the remaining randomness (corresponding to
$dT - \ell_v$ requests) is not used. This unused randomness is both present in
the uncompressed representation $R$ and in its compressed counterpart $R'$ and
is represented as is in $R'$, thus corresponding to $\sum_{v\in V} (dT -
\ell_v)\log\Delta$ bits.


\subsubsection{Compression}
In this section, we show that, if $R$ represents an execution terminating and
returning a {\em non expanding} graph $H$, the corresponding encoding according
to the scheme presented in the previous section uses $ndT\log\Delta -
\Omega(\log n)$. In more detail, we apply our encoding scheme to any subset
$S\subset V$ that is not an ``$\freq$-expander'' in the graph $H$ returned by
\ALG.

The proof of compression proceeds by carefully bounding the costs of the
compressed representation $R'$ and comparing them with their counterparts in
the uncompressed representation $R$.  We first show that the additive costs
(with respect to $R$) of representing the non-expanding set $S$ \eqref{reps}
and the subset of accepted requests with destinations in $V - S$ \eqref{repcut}
are more than compensated by the compression achieved in the representation of
accepted requests with destinations in $S$ \eqref{reprandacc}, with total
savings $\Omega(ds\log\frac{n}{s})$.  This first step corresponds to bounding
the partial cost \eqref{reps} + \eqref{repcut} + \eqref{reprandacc}.

If this is intuitively the key argument, it is neglecting the fact that we now
need to identify the subset of requests originating from $S$ that are accepted
\eqref{repaccs}. For each node, this cost depends on the number of failures and
in general cannot be compensated by the aforementioned savings. To this
purpose, we need to exploit the further property that, for each node, failures
have destinations that, for each round $t$, correspond to an $\bigO(1/c)$
fraction of the vertices. Compressing the destinations of these requests allows
to compensate the aforementioned cost almost entirely. This second step
corresponds to bounding the partial cost \eqref{repaccs} + \eqref{repcrit} +
\eqref{reprandrej}.


\paragraph{Bounding \eqref{reps} + \eqref{repcut} + \eqref{reprandacc}.} We
begin by bounding the overall compressed cost of representing the destinations
of accepted requests from nodes in $S$, as well as the corresponding savings
with respect to $R$. This is a crucial contribution, which depends on the
expansion properties of the underlying graph $G$.

\begin{claim}\label{cl:sav_accepted}
Under the hypotheses of Theorem \ref{thm:main-expanders}, the overall cost of
representing the subset of accepted requests from nodes in $S$ is at most
\begin{equation}\label{eq:sav_accepted}
\sum_{v\in S}(1 - \freq_v)\nreq\log ((1 - \out_v)\Delta) 
+ \sum_{v\in S}\freq_v\nreq\log\Delta\le sd\log\Delta 
- \frac{1 - \freq}{2}sd\log\frac{n}{s} + 2\freq ds \,,
\end{equation}
thus the saving is at least
\begin{equation*}
\frac{1 - \freq}{2}sd\log\frac{n}{s} - 2\freq ds
\end{equation*}
bits over the uncompressed representation.
\end{claim}
\begin{proof}
We directly give a lower bound to the savings achieved with respect to the
uncompressed representation, namely, we prove that
\[
sd\log\Delta - \left(\sum_{v\in S}(1 - \freq_v)\nreq\log ((1 - \out_v)\Delta) 
+ \sum_{v\in S}\freq_v\nreq\log\Delta\right)
\ge \frac{1 - \freq}{2}ds\log\frac{n}{s} - 2\freq ds \, ,
\]
whence \eqref{eq:sav_accepted} immediately follows. 
First of all we have
\begin{align*}
& sd\log\Delta - \left(\sum_{v\in S}(1 - \freq_v)\nreq\log ((1 - \out_v)\Delta) 
  + \sum_{v\in S}\freq_v\nreq\log\Delta\right)\\
& = \nreq\sum_{v\in S}(1 - \freq_v)\log\Delta - \nreq\sum_{v\in S}(1 - \freq_v)\log((1 - \out_v)\Delta) 
= \nreq\sum_{v\in S}(1 - \freq_v)\log\frac{1}{1 - \out_v} \, .
\end{align*}
Next, we consider two cases.

\paragraph{Case $s < \alpha\Delta$.} In this case, we use the following
observation, that is obviously true, since $\out_v s$ is exactly the number of
$v$'s edges that have the other end-point in $V - S$

\begin{obs}\label{obs:s_small}
\[
1 - \out_v\le\frac{s}{\Delta} \, .
\]
\end{obs}
In this case
\begin{align*}
& \nreq\sum_{v\in S}(1 - \freq_v)\log\frac{1}{1 - \out_v}
\ge\nreq\sum_{v\in S}(1 - \freq_v)\log\frac{\Delta}{s} 
= (1 - \freq)sd\log\frac{\Delta}{s} 
> \frac{1 - \freq}{2}sd\log\frac{n}{s} \, ,
\end{align*}
where we used Observation \ref{obs:s_small} to write the first 
inequality, while the last inequality follows since in this case
\[
\frac{\Delta}{s} > \frac{1}{\alpha} = \frac{n}{\Delta} \, ,
\]
which in turn implies
\[
\left(\frac{\Delta}{s}\right)^2 > \frac{n}{s} \, .
\]

\paragraph{The case $\alpha\Delta\le s\le n/2$.} In this case, the proof is a
bit more articulated. To begin, we can write
\begin{align*}
& \sum_{v\in S}(1 - \freq_v)\log\frac{1}{1 - \out_v} 
= -\sum_{v\in S}(1 - \freq_v)\log(1 - \out_v) 
= -(1 - \freq)s\sum_{v\in S}\frac{1 - \freq_v}{(1 - \freq)s}\log(1 - \out_v)\\
& \ge -(1 - \freq)s\log\frac{\sum_{v\in S}(1 - \freq_v)(1 - \out_v)}{(1 
	- \freq)s}
\ge-(1 - \freq)s\log\frac{\sum_{v\in S}(1 - \out_v)}{(1 - \freq)s} 
= (1 - \freq)s\log\frac{1 - \freq}{1 - \out} \, .
\end{align*}
Here, to derive the third inequality we used Jensen's inequality on $\sum_{v\in
S}\frac{1 - \freq_v}{(1 - \freq)s}\log(1 - \out_v)$, which is a convex
combination of values of a concave function. 
Next, we use the following simple claim. 

\begin{claim}\label{cl:s_big}
\[
1 - \out \, \le \, \frac{s}{n} + \frac{\lambda}{\Delta} \, .
\]
\end{claim}

\begin{proof}
From the definition of $\out_v$ we have 
\[
e(S, S) = \sum_{v\in S}(1 - \out_v)\Delta = (1 - \out)s\Delta \, .
\]
The claim then follows immediately from Lemma \ref{le:exp_mixing_lemma}. 
\end{proof}

Next, using the above derivations and Claim \ref{cl:s_big}, we can write:
\begin{align*}
	&\nreq\sum_{v\in V}(1 - \freq_v)\log\frac{1}{1 - \out_v}\ge (1 - 
	\freq)ds\log\frac{1 - \freq}{1 - \out}\ge(1 - \freq)ds\log\frac{(1 - 
	\freq)n\Delta}{\lambda n + \Delta s}\ge (1 - \freq)sd\log\frac{n}{s} - 
	2\freq ds \, .
\end{align*}
To prove the last inequality, we note that 
\[
	\frac{(1 - \freq)n\Delta}{\lambda n + \Delta s}\ge 
	\frac{n}{s}\cdot\frac{1 - \freq}{1 + \freq}\, ,
\]
whenever 
\[
	\frac{1}{s}\le (1 + \freq)\frac{\Delta}{s\Delta + \lambda n} \, ,
\]
which happens if $\lambda n\le \freq s\Delta$. Since we are assuming 
$s\ge\alpha\Delta$, this is certainly true if 
$\lambda\le\freq\alpha^2\Delta$. Substituting back into $\log\frac{(1 - 
\freq)n\Delta}{\lambda n + \Delta s}$ straightforwardly yields the 
result. 
\end{proof}

We can now bound \eqref{reps} + \eqref{repcut} +  
\eqref{reprandacc}. First notice that 
\[
	\eqref{reps} = 2\log s + \log {n \choose s}\le 3s\log\frac{n}{s} \, ,
\]
since we are assuming $\alpha^2 n \leq s \le n/2$ and it holds $\log {n \choose
s} \leq s \log (ne/s)$.

As for \eqref{repcut} we have
\begin{equation*}
	2\sum_{v\in S}\log\freq_v d = 2\log\prod_{v\in S}(\freq_v 
	d)
	\le 2\log\left(\frac{\sum_{v\in S}\freq_v d}{s}\right)^s = 2s\log 
	\freq d\, ,
\end{equation*}
where the second inequality follows from the AM-GM inequality 
\cite{steele2004cauchy}, while the last equality follows from the 
definition of $\freq$. We further have
\begin{align*}
	&\sum_{v\in S}\log\binom{d}{\freq_v 
	d}\le d\sum_{v\in S}\freq_v\log\frac{e}{\freq_v} = \freq ds\log e + 
	\sum_{v\in S}\freq_v\log\frac{1}{\freq_v}\le\freq ds\log e + \freq 
	s\log\frac{1}{\freq} \, .
\end{align*}
Here, the second equality follows since $\sum_{v\in S}\freq_v = \freq 
s$ by definition, while the third inequality follows since the optimum 
of the following problem
\begin{align*}
	&\max g(x_1, ... , x_k) = \sum_{i=1}^k x_i\log\frac{1}{x_i}\\
	&\sum_{i=1}^k x_i = A\\
	&x_i\ge 0\, ,
\end{align*}
is achieved when $x_1 = \ldots = x_k = A/k$.
So, overall we have
\begin{align}\label{eq:partial1}
	&\eqref{reps} + \eqref{repcut} + \eqref{reprandacc}\le 
	3s\log\frac{n}{s} + \underbrace{2s\log\freq d + \freq ds\log e + \freq 
	s\log\frac{1}{\freq}}_{*} + ds\log\Delta - \frac{1 - \freq}{2}ds\log\frac{n}{s} + 2\freq ds\nonumber\\
	&\le 3s\log\frac{n}{s} + ds\log\Delta - \frac{1 - 13\freq}{2} ds\log\frac{n}{s} + 2\freq ds\, ,
\end{align}
where the last inequality holds, since each of the starred terms is at 
most $2\freq ds\log\frac{n}{s}$, whenever $s\le n/2$ and 
$d\ge\frac{1}{2}\log\frac{1}{\freq}$.

\paragraph{Bounding \eqref{repaccs} + \eqref{repcrit} + \eqref{reprandrej}.} 
For $\eqref{repaccs}$ we have
\begin{align*}
	&\eqref{repaccs} = \sum_{v\in S}\left(2\log\ell_v + 
	\log\binom{\ell_v}{d}\right)\le a(\ell_v - d) + \frac{1}{4}d\, ,
\end{align*}
where $a$ is an absolute constant and where, to derive the second inequality,
we used the following fact:

\begin{claim}\label{cl:tech2}
For every $b$ there is a sufficiently large $a$ such that, for every $d$ and
every $\ell > d$ we have
\[ 
\log {\ell \choose d} \leq a \cdot(\ell - d ) + b d \, .
\]
\end{claim}

As for \eqref{repcrit}, the definition of critical node at round $t$ implies
that each critical node at round $t$ is receiving more than $cd/2$ of its
incoming requests from nodes in $S$. As a consequence, we get
\[
\sum_{v\in S}\rc_t(v) > \frac{cd}{2}c_t \, ,
\]

For the first term in \eqref{repcrit} this implies
\begin{align*}
	&2\sum_{t=1}^T\log c_t\le 
	2\sum_{t=1}^T\log\left(\frac{2}{cd}\sum_{v\in S}\rc_t(v)\right) < 
	\frac{4}{cd}\sum_{t=1}^T\sum_{v\in 
	S}\rc_t(v)\le\frac{4}{cd}\sum_{v\in S}(\ell_v - d) \, ,
\end{align*}
where to derive the last inequality we exchanged the order of summation 
and used the fact that $\sum_{t=1}^T\rc_t(v)\le \ell_v - d$, while 
for the for the second term in \eqref{repcrit} we have
\begin{align*}
	&\log\binom{n}{c_t}\le c_t\log\frac{en}{c_t}\le\frac{2}{cd}\sum_{v\in 
	S}\rc_t(v)\log\frac{en}{c_t}\le\sum_{v\in 
	S}\rc_t(v)\log\frac{2n}{c\cdot c_t}.
\end{align*}
Here, to derive the third inequality we used the following

\begin{claim}\label{cl:tech1}
\[
\log\left(\frac{en}{c_t}\right)^{\frac{2}{cd}}\le\log\frac{2n}{c\cdot c_t}\, ,
\]
whenever $c$ is large enough that $d\ge\frac{2}{c}\log\frac{ce}{2}$.
\end{claim}
\begin{proof}
The proof follows from simple calculus, recalling that the definition 
of critical node implies that there are at most $n/c$ of them at any 
round $t$.
\end{proof}

At this point, we give an upper bound to $\eqref{repaccs} + \eqref{repcrit} + 
\eqref{reprandrej}$. Let $\gamma = 1 + a + \frac{4}{cd}$. We have
\begin{align}\label{eq:partial2}
	&\eqref{repaccs} + \eqref{repcrit} + 
	\eqref{reprandrej}\le\gamma\sum_{v\in S}\left((\ell_v - d) + 
	\frac{1}{4}d + \sum_{t=1}^T
	\rc_t(v)\log\frac{2n}{c\cdot c_t} + \rss(v) \cdot \log 
	\frac{2n}{c} + \sum_{t=1}^T \rc_t(v) \cdot \log c_t 
	\right)\nonumber\\
	& = \gamma\sum_{v\in S}(\ell_v - d) + \frac{1}{4}ds + \sum_{v\in S}\left(\rss(v) \cdot \log 
	\frac{2n}{c} + \sum_{t=1}^T\rc_t(v)\log\frac{2n}{c}\right)\nonumber\\
	& \le \gamma\sum_{v\in S}(\ell_v - d) + \frac{1}{4}ds + 
	\log\Delta\sum_{v\in S}(\ell_v - d) - \frac{1}{2}\sum_{v\in 
	S}(\ell_v - d)\log c\nonumber\\
	&\le\log\Delta\sum_{v\in S}(\ell_v - d) + \frac{1}{4}ds \, .
\end{align}
Here, in the third inequality we used $\Delta = \alpha n$ and we considered
$c\ge (2/\alpha)^2$, so that $\Delta\ge 2n/\sqrt{c}$, while in the last
inequality we used the fact that $\gamma\le\log\frac{c}{2}$ for sufficiently
large $c$.  As a result, the total number of bits to encode the executions of
nodes in $S$ is as follows (recall that we use $(n - s)dT\log\Delta	$ bits for
vertices in $V - S$).
\begin{equation}\label{eq:total}
	\eqref{reps} + \eqref{repcut} +  \eqref{reprandacc} + 
	\eqref{repaccs} + \eqref{repcrit} + 
	\eqref{reprandrej}\le 3s\log\frac{n}{s} + ds\log\Delta - \frac{1 - 13\freq}{2} ds\log\frac{n}{s} + 2\freq ds
	 + \log\Delta\sum_{v\in S}(\ell_v - d) + \frac{1}{4}ds \, .
\end{equation}
To this cost, we should also add the randomness that was not used, 
which is exactly $(dT - \ell_v)\log\Delta$ for the generic node $v$. 
Our savings are then 
\begin{align*}
	&\mbox{Savings}\ge dsT\log\Delta - \left(3s\log\frac{n}{s} + ds\log\Delta - \frac{1 - 13\freq}{2} ds\log\frac{n}{s} + 2\freq ds
	 + \log\Delta\sum_{v\in S}(dT - d) + \frac{1}{4}ds\right)\\
	& = - 3s\log\frac{n}{s} + \frac{1 - 13\freq}{2} ds\log\frac{n}{s} - 
	\left(\frac{1}{4} + 2\freq\right)ds \, ,
\end{align*}
Finally, the expression above is $\Omega(\log n)$, as soon as $\freq$ is a
sufficiently small (absolute) constant.\footnote{E.g., $\freq\le 1/51$ will
suffice.}


